TV-based Deep 3D Self Super-Resolution for fMRI

While functional Magnetic Resonance Imaging (fMRI) offers valuable insights into cognitive processes, its inherent spatial limitations pose challenges for detailed analysis of the fine-grained functional architecture of the brain. More specifically, MRI scanner and sequence specifications impose a trade-off between temporal resolution, spatial resolution, signal-to-noise ratio, and scan time. Deep Learning (DL) Super-Resolution (SR) methods have emerged as a promising solution to enhance fMRI resolution, generating high-resolution (HR) images from low-resolution (LR) images typically acquired with lower scanning times. However, most existing SR approaches depend on supervised DL techniques, which require training ground truth (GT) HR data, which is often difficult to acquire and simultaneously sets a bound for how far SR can go. In this paper, we introduce a novel self-supervised DL SR model that combines a DL network with an analytical approach and Total Variation (TV) regularization. Our method eliminates the need for external GT images, achieving competitive performance compared to supervised DL techniques and preserving the functional maps.

==> stuff.tex <==
OPNEURO f=1.25
TRAINING MSE NEAREST 0.0006111086340238886 PSNR 74.00235817503601 SSIM 0.9323678663104409
TRAINING MSE SPLINE 0.0003346795106584481 PSNR 80.02337168655644 SSIM 0.9559046901399173
f=1.25
VALIDATION MSE NEAR 0.0005573609043862661 PSNR 74.92297584618734 SSIM 0.9350661355583112
VALIDATION MSE SPLINE 0.00030308837435569864 PSNR 81.01486130440479 SSIM 0.9570730328746775

f=1.5
VALIDATION MSE NEAR 0.0008520504133650188 PSNR 70.6786486226925 SSIM 0.9076577147805709
VALIDATION MSE SPLINE 0.0005226202970184167 PSNR 75.56655367096909 SSIM 0.9334265155294655

f=1.75
VALIDATION MSE NEAR 0.0012431115031197493 PSNR 66.90137765633881 SSIM 0.8711931045113172
VALIDATION MSE SPLINE 0.0007774283319069953 PSNR 71.59519095771083 SSIM 0.9072611589271883

f=2
VALIDATION MSE NEAR 0.0010623417529777661 PSNR 68.4727960663199 SSIM 0.8874385501931912
VALIDATION MSE SPLINE 0.0011801377643173541 PSNR 67.42124097897761 SSIM 0.8729468551734382

Table before correcting
& &PSNR & SSIM& PSNR & SSIM& PSNR & SSIM& PSNR & SSIM& PSNR & SSIM\\
         \midrule
         1.857&1.25 & 78.1602 & 0.9446 & 86.2074 & 0.9731 & 0& 0& 84.5387 &0.9648& 85.8236 & 0.9713\\
         2.25&1.5 & 75.0657 & 0.9265 & 82.4568 & 0.9607 & 0& 0& 79.8466 &0.9503 &80.0356 & 0.9546\\
         2.62&1.75 & 73.5425 & 0.9169 & 78.6634 & 0.9460 & 0& 0& 75.7364 &0.9273& 76.7245 & 0.9368\\
         3&2 & 69.5865 & 0.8855 & 76.3187 & 0.9375 & 76.2697& 0.9332& 73.1682 & 0.9104 &73.4461&0.9192\\


%SUPER
% 0 & 86.2074 &        0.9726 \\
% 1 & 82.4568 &        0.9607 \\
% 2 & 78.6634 &        0.9439 \\

% EUGENIO
% 0 & 86.2074 &        0.9731 \\
% 1 & 82.4568 &        0.9607 \\
% 2 & 78.6634 &        0.9460 \\

% NO TV (DIP)
% 0 & 84.5387 &0.9648 \\
% 1 & 79.8466 &0.9503 \\
% 2 & 75.7364 &0.9273 \\

% TV values at TV_weight= 0.007
% 1.25 & 85.8236 &        0.9713 \\
% 1.5 & 80.0356 &        0.9546 \\
% 1.75 & 76.7245 &        0.9368 \\
% 0 &  0.00018738 & 85.8236 &   142 &        0.9713 &    137 \\
% 1 &  0.00033427 & 80.0356 &   237 &        0.9546 &    237 \\
% 2 &  0.00046548 & 76.7245 &   127 &        0.9368 &    127 \\

% 1.25
% TRAINING MSE 0.0004394630825472132 PSNR 77.29956843122054 SSIM 0.942010444768988
% VALIDATION MSE 0.00040322163524261333 PSNR 78.16024183810852 SSIM 0.9446348476191807
% TEST MSE 0.0005110159701216001 PSNR 75.79109715564775 SSIM 0.9356062400765366
% 1.5
% TRAINING MSE 0.0006104443795254157 PSNR 74.01323374992432 SSIM 0.922639025173628
% VALIDATION MSE 0.0005494634034801645 PSNR 75.06568386010585 SSIM 0.9265478951934136
% TEST MSE 0.0007269110019803955 PSNR 72.26706506108246 SSIM 0.9134669223543675
% 1.75
% TRAINING MSE 0.00070240539520655 PSNR 72.60999834570147 SSIM 0.9123410323829364
% VALIDATION MSE 0.0006398678947065143 PSNR 73.54248817438037 SSIM 0.9169173188109405
% TEST MSE 0.0008396883911041479 PSNR 70.82479697921951 SSIM 0.902144193513344
% 2
% TRAINING MSE 0.001071907612785116 PSNR 68.38315402150853 SSIM 0.8780404173231907
% VALIDATION MSE 0.0009503789514504502 PSNR 69.58649756644019 SSIM 0.8854631258948757
% TEST MSE 0.0012890047620647475 PSNR 66.53884860644985 SSIM 0.8646381615511025
